Joint Motion, Angle, and Range Estimation in Near-Field under Array Calibration Imperfections

Ultra-massive multiple-input multiple-output MIMO (UM-MIMO) leverages large antenna arrays at high frequencies, transitioning communication paradigm into the radiative near-field (NF), where spherical wavefronts enable full-vector estimation of both target location and velocity. However, location and motion parameters become inherently coupled in this regime, making their joint estimation computationally demanding. To overcome this, we propose a novel approach that projects the received two-dimensional space-time signal onto the angle-Doppler domain using a two-dimensional discrete Fourier transform (2D-DFT). Our analysis reveals that the resulting angular spread is centered at the target's true angle, with its width determined by the target's range. Similarly, transverse motion induces a Doppler spread centered at the true radial velocity, with the width of Doppler spread proportional to the transverse velocity. Exploiting these spectral characteristics, we develop a low-complexity algorithm that provides coarse estimates of angle, range, and velocity, which are subsequently refined using one-dimensional multiple signal classification (MUSIC) applied independently to each parameter. The proposed method enables accurate and efficient estimation of NF target motion parameters. Simulation results demonstrate a normalized mean squared error (NMSE) of -40 dB for location and velocity estimates compared to maximum likelihood estimation, while significantly reducing computational complexity.

==> acronym.tex <==
\usepackage{etoolbox}
\makeatletter
\newif\ifAC@uppercase@first%
\def\Aclp#1{\AC@uppercase@firsttrue\aclp{#1}\AC@uppercase@firstfalse}%
\def\AC@aclp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acl{#1}s%
	\fi%
}%
\def\Acp#1{\AC@uppercase@firsttrue\acp{#1}\AC@uppercase@firstfalse}%
\def\AC@acp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@ac{#1}s%
	\fi%
}%
\def\Acfp#1{\AC@uppercase@firsttrue\acfp{#1}\AC@uppercase@firstfalse}%
\def\AC@acfp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acf{#1}s%
	\fi%
}%
\def\Acsp#1{\AC@uppercase@firsttrue\acsp{#1}\AC@uppercase@firstfalse}%
\def\AC@acsp#1{%
	\ifcsname fn@#1@PL\endcsname%
	\ifAC@uppercase@first%
	\expandafter\expandafter\expandafter\MakeUppercase\csname fn@#1@PL\endcsname%
	\else%
	\csname fn@#1@PL\endcsname%
	\fi%
	\else%
	\AC@acs{#1}s%
	\fi%
}%
\edef\AC@uppercase@write{\string\ifAC@uppercase@first\string\expandafter\string\MakeUppercase\string\fi\space}%
\def\AC@acrodef#1[#2]#3{%
	\@bsphack%
	\protected@write\@auxout{}{%
		\string\newacro{#1}[#2]{\AC@uppercase@write #3}%
	}\@esphack%
}%
\def\Acl#1{\AC@uppercase@firsttrue\acl{#1}\AC@uppercase@firstfalse}
\def\Acf#1{\AC@uppercase@firsttrue\acf{#1}\AC@uppercase@firstfalse}
\def\Ac#1{\AC@uppercase@firsttrue\ac{#1}\AC@uppercase@firstfalse}
\def\Acs#1{\AC@uppercase@firsttrue\acs{#1}\AC@uppercase@firstfalse}
\robustify\Aclp
\robustify\Acfp
\robustify\Acp
\robustify\Acsp
\robustify\Acl
\robustify\Acf
\robustify\Ac
\robustify\Acs
\makeatother


%%%%%%%%%%%%%%%%%%%%%% Predefined
\acrodef{DoF}[DoF]{degrees of freedom}
\acrodef{URA}[URA]{uniform rectangular array}
\acrodef{USA}[USA]{uniform square array}
\acrodef{EBRD}[EBRD]{effective beamfocusing Rayleigh distance}
\acrodef{ULA}[ULA]{uniform linear array}
\acrodef{BS}[BS]{base station}
\acrodef{MIMO}[MIMO]{multiple-input multiple-output}
\acrodef{UM}[UM]{ ultra-massive}
\acrodef{LoS}[LoS]{line-of-sight }
\acrodef{HBF}[HBF]{hybrid beamforming}
\acrodef{IQ}[IQ]{in-phase and quadrature-phase}
\acrodef{RF}[RF]{radio frequency}
\acrodef{LDMA}[LDMA]{location division multiple access}
\acrodef{SDMA}[SDMA]{spatial division multiple access}
\acrodef{ERD}[ERD]{effective Rayleigh distance}
\acrodef{BAND}[BAND]{bandwidth-aware near-field distance}
\acrodef{UCA}[UCA]{uniform circular array}
\acrodef{CAP}[CAP]{continuous aperture}
\acrodef{SPD}[SPD]{spatially discrete}
\acrodef{NMSE}[NMSE]{normalized mean square error}
\acrodef{UE}[UE]{user equipment}
\acrodef{USW}[USW]{uniform spherical wave}
\acrodef{CS}[CS]{compressed sensing}
\acrodef{DFT}[DFT]{discrete Fourier transform}
\acrodef{BF-SOMP}[BF-SOMP]{beam-focused simultaneous orthogonal matching pursuit}
\acrodef{OFDM}[OFDM]{Orthogonal Frequency Division Multiplexing}
\acrodef{CSI}[CSI]{channel state information}
\acrodef{SOMP}[SOMP]{simultaneous orthogonal matching pursui}
\acrodef{SE}[SE]{spectral efficiency}
\acrodef{FFT}[FFT]{fast Fourier transform}
\acrodef{IFFT}[IFFT]{inverse fast Fourier transform}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{GBR}[GBR]{guaranteed bit-rate}
\acrodef{GFDM}[GFDM]{generalized orthogonal frequency division multiplexing}
\acrodef{RSRP}[RSRP]{reference signal received power}
\acrodef{CSI-RSRP}[CSI-RSRP]{CSI-reference signal received power}
\acrodef{5G}[5G]{fifth generation}
\acrodef{4G}[4G]{fourth generation}
\acrodef{SISO}[SISO]{single-input single-output}
\acrodef{GCoMP}[GCoMP]{generalized CoMP}
\acrodef{CU}[CU]{central unit}
\acrodef{DU}[DU]{distributed unit}
\acrodef{RU}[RU]{remote unit}
\acrodef{FH}[FH]{fronthaul}
\acrodef{TBS}[TBS]{terrestrial base station}
\acrodef{IoE}[IoE]{Internet of Everything}
\acrodef{SI}[SI]{self-interference}
\acrodef{FBS}[FBS]{flying base station}
\acrodef{PLS}[PLS]{physical layer security}
\acrodef{PRB}[PRB]{physical resource block}
\acrodef{PSK}[PSK]{phase-shift keying}
\acrodef{QAM}[QAM]{quadrature amplitude modulation}
\acrodef{ostbc}[OSTBC]{orthogonal space time block codes}
\acrodef{OOBE}[OOBE]{out-of-band emission}
\acrodef{svd}[SVD]{singular value decomposition}
\acrodef{MAC}[MAC]{medium access control}
\acrodef{PHY}[PHY]{physical}
\acrodef{THz}[THz]{terahertz}
\acrodef{RIS}[RIS]{reconfigurable intelligent surface}
\acrodef{QoS}[QoS]{quality-of-service}
\acrodef{HO}[HO]{handover}
\acrodef{MBB}[MBB]{\textit{Make-Before-Break}}
\acrodef{RACH}[RACH]{\textit{Random Access Channel}}
\acrodef{eMTC}[eMTC]{\textit{enhanced machine type communication}}
\acrodefplural{GBR}[GBR]{guaranteed bit rate}
\acrodef{RB}[RB]{resource block}
\acrodef{PPP}[PPP]{Poisson point process}
\acrodef{ZF}[ZF]{zero-forcing}
\acrodef{RSSI}[RSSI]{received signal strength indicator}
\acrodef{CIR}[CIR]{channel impulse response}
\acrodef{CFR}[CFR]{channel frequency response}
\acrodef{CP}[CP]{cyclic prefix}
\acrodef{ISI}[ISI]{inter-symbol interference}
\acrodef{UAV}[UAV]{unmanned aerial vehicle}
\acrodef{ISD}[ISD]{inter-site distance}
\acrodef{OFDM}[OFDM]{orthogonal frequency-division multiplexing}
\acrodef{BER}[BER]{bit error rate}
\acrodef{CSF}[CSF]{channel shortening filter}
\acrodef{AWGN}[AWGN]{additive white Gaussian noise}
\acrodef{TDD}[TDD]{time-division duplex}
\acrodef{FDD}[FDD]{frequency-division duplex}
\acrodef{SNR}[SNR]{signal-to-noise ratio}
\acrodef{MSSNR}[MSSNR]{maximum shortening signal-to-noise ratio}
\acrodef{PSD}[PSD]{power spectral density}
\acrodef{QPSK}[QPSK]{Quadrature Phase Shift Keying}
\acrodef{MMSE}[MMSE]{ minimum mean-squared error}
\acrodef{Rx}[Rx]{receiver}
\acrodef{Tx}[Tx]{transmitter}
\acrodef{TRCPR}[TRCPR]{\ac{Tx}-\ac{Rx} channel-based phase rotation}
\acrodef{TOCPR}[TOCPR]{\ac{Tx}-only channel-based phase rotation}
\acrodef{ML}[ML]{maximum likelihood}
\acrodef{SDCO}[SDCO]{spatially Distributed constellation obfuscation}
\acrodef{PDF}[PDF]{probability density function}
\acrodef{mmWave}[mmWave]{millimeter wave}
\acrodef{SER}[SER]{symbol error rate}
\acrodef{MISO}[MISO]{multiple-input single-output}
\acrodef{FD}[FD]{full-duplex}
\acrodef{AN}[AN]{artificial noise}
\acrodef{SC}[SC]{secrecy capacity}
\acrodef{IBFD}[IBFD]{in-band full-duplex}
\acrodef{KPI}[KPI]{key performance indicator}
\acrodef{VR}[VR]{virtual reality}
\acrodef{AR}[AR]{augmented reality}
\acrodef{6G}[6G]{sixth generation}
\acrodef{RF}[RF]{radio frequency}
\acrodef{PZ}[PZ]{protected zone}
\acrodef{SIC}[SIC]{\ac{SI} cancellation}
\acrodef{SA}[SA]{simulated annealing }
\acrodef{AI}[AI]{artificial intelligence}
\acrodef{BCD}[BCD]{block coordinate descent}
\acrodef{EE}[EE]{energy efficiency}
\acrodef{MUSIC}[MUSIC]{multiple signal classification}
\acrodef{NF}[NF]{near-field}
\acrodef{AD}[AD]{angle-Doppler}
\acrodef{FF}[FF]{far-field}
\acrodef{CPI}[CPI]{coherent processing interval}
\acrodef{RCS}[RCS]{radar cross section}
\acrodef{AoA}[AoA]{angle of arrival}
\acrodef{D}[D]{dimensional}




